Can humans teach machines to code?

The goal of inductive program synthesis is for a machine to automatically generate a program from user-supplied examples. A key underlying assumption is that humans can provide sufficient examples to teach a concept to a machine. To evaluate the validity of this assumption, we conduct a study where human participants provide examples for six programming concepts, such as finding the maximum element of a list. We evaluate the generalisation performance of five program synthesis systems trained on input-output examples (i) from non-expert humans, (ii) from a human expert, and (iii) randomly sampled. Our results suggest that non-experts typically do not provide sufficient examples for a program synthesis system to learn an accurate program.

==> D-popper.tex <==
\section{Learning settings}
We impose a functional restriction to compensate for the lack of negative examples. 

==> figures.tex <==

\begin{figure}
\begin{minipage}{\textwidth}
\includegraphics[width=9cm]{figures/nexamples.png}
\end{minipage}
\caption{Number of examples provided by participants.\label{fig:n_exs}
}

\begin{minipage}{\textwidth}
\includegraphics[width=9cm]{figures/length_lists.png}
\end{minipage}
\caption{Length of lists provided by participants.\label{fig:list_length}
}

\begin{minipage}{\textwidth}
\includegraphics[width=9cm]{figures/element_values.png}
\end{minipage}
\caption{Values of elements provided by participants.\label{fig:element_values}
}
\end{figure}
